Beyond MLE: Convex Learning for Text Generation

Maximum likelihood estimation (MLE) is a statistical method used to estimate the parameters of a probability distribution that best explain the observed data. In the context of text generation, MLE is often used to train generative language models, which can then be used to generate new text. However, we argue that MLE is not always necessary and optimal, especially for closed-ended text generation tasks like machine translation. In these tasks, the goal of model is to generate the most appropriate response, which does not necessarily require it to estimate the entire data distribution with MLE. To this end, we propose a novel class of training objectives based on convex functions, which enables text generation models to focus on highly probable outputs without having to estimate the entire data distribution. We investigate the theoretical properties of the optimal predicted distribution when applying convex functions to the loss, demonstrating that convex functions can sharpen the optimal distribution, thereby enabling the model to better capture outputs with high probabilities. Experiments on various text generation tasks and models show the effectiveness of our approach. It enables autoregressive models to bridge the gap between greedy and beam search, and facilitates the learning of non-autoregressive models with a maximum improvement of 9+ BLEU points. Moreover, our approach also exhibits significant impact on large language models (LLMs), substantially enhancing their generative capability on various tasks. Source code is available at \url{https://github.com/ictnlp/Convex-Learning}.

==> Figures/COMET_PPL.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/COMET_PPL_fig.pdf}
    \caption{Translation quality (COMET Score) and generation fluency (Perplexity) of different NAT models as the exponent ($k$) varies on WMT14 EN-DE test set.}
    \label{fig:COMET&NLL}
\end{figure}

==> Figures/Shape.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.55\linewidth]{Figures/Shape_fig.pdf}
    \caption{Translation quality (BLEU) of autoregressive model as beam size varies on WMT14 EN$\leftrightarrow$DE test set.}
    \label{fig:Shape}
\end{figure}
